Equilibrium of Blockchain Miners with Dynamic Asset Allocation

We model and analyze blockchain miners who seek to maximize the compound return of their mining businesses. The analysis of the optimal strategies finds a new equilibrium point among the miners and the mining pools, which predicts the market share of each miner or mining pool. The cost of mining determines the share of each miner or mining pool at equilibrium. We conclude that neither miners nor mining pools who seek to maximize their compound return will have a financial incentive to occupy more than 50% of the hash rate if the cost of mining is at the same level for all. However, if there is an outstandingly cost-efficient miner, then the market share of this miner may exceed 50% in the equilibrium, which can threaten the viability of the entire ecosystem.

==> A0_asymptotic.tex <==
\section{Proof for the approximation in Section \ref{OptimalF}}

This section gives proofs of the approximation formula for $\E[\log(1+X_i)]$.
First, we can write the optimal $f$ explicitly:

\begin{align*}
\E[\log(1+ X_i)] &= p_i \log(1 + (1-f) r + f u_i) + (1-p_i)\log(1+ (1-f)r + f d_i)
\end{align*}
%\frac{M_{i}\,\log\left(-\frac{\left(M_{i}\,f-M_{i}\right)\,r+\left(M_{i}\,c-B\right)\,f-M_{i}}{M_{i}}\right)}{M_{i}+M_{-i}} +\frac{M_{-i}\,\log\left(\left(1-f\right)\,r-c\,f+1\right)}{M_{i}+M_{-i}}
for
$$
p_i = \frac{M_i}{M_i + M_{-i}},
$$
$$
u_i = \frac{B}{M_i} - c,
$$
and
$$
d_i = -c.
$$
By a straight-forward calculus we obtain
\begin{align*}
     f_\text{max} & =\frac{M_{i}\,\left(r+1\right)\,\left( (M_i + M_{-i}) (c+r)-B\right)}{\left(M_{-i}+M_{i}\right)\,\left(r+c\right)\,\left(M_{i}\,(r+c)-B\right)}.
\end{align*}


Let
$$
\mu = \frac{B}{M_i + M_{-i}} -  c.
$$
We approximate $f_\text{max}$ and $\E[\log(1+X_i)]$ when $\mu$ is small.
By eliminating $M_i$ we obtain
\begin{align*}
f_\text{max} &= \frac{ \left(B- M_{-i}\,(\mu+c) \right)\,\left(r+1\right)\,\left(\mu-r\right)}{\left(c+r\right)\,\left(M_{-i}\,(\mu + c) (c + r) +B\,(\mu - r)\right)},
\end{align*}
so we have this lemma.
\begin{lemma}
If $0 < r < \mu$, then
\begin{align*}
    f_\text{max} &< \frac{B (r+1) (\mu -r)}{M_{-i} c^3}.
\end{align*}
\end{lemma}

We are interested in $f$ that maximizes the log-return, so we assume $f = O(\mu)$ as $r, \mu \to 0$.


\begin{prop}
Assuming $0< r <\mu$ and $f = O(\mu)$ as $r, \mu \to 0$, we have
$$
\E[\log(1+X_i)] = \E[X_i] - \frac{\E[X_i^2]}{2} + O(\mu^3)
$$
as $r, \mu \to 0$.
\end{prop}
\begin{proof}
Since $\log(1+x) -( x - \frac{x^2}{2}) < \frac{x^3}{3}$ for all $x> -1$, we have
$\E[\log(1+X_i)] - (\E[X_i] - \frac{\E[X_i^2]}{2}) < \E[X_i^3],$
so it suffices to show $\E[X_i^3]= O(\mu^3)$.
Eliminating $M_i$, we have $p_i = 1- \frac{M_{-i}(\mu + c)}{B}$ and $1-p_i = \frac{M_{-i}(\mu + c)}{B}$.
Since $f = O(\mu)$ and $0 < r< \mu$,
there exists $C=C(c, M_{-i})$ that satisfies
\begin{align*}
    \E[X_i^3] &= p_i ( (1-f) r + f u_i)^3 + (1-p_i) ( (1-f)r + f d_i)^3\\
    &\le  C \mu^3
\end{align*}
for sufficiently small $\mu$.
%
%Thus we have 
%$$
%\E[\log(1+X_i)] = \E[X_i] - \frac{\E[X_i^2]}{2} + O(\mu^3).
%$$
\end{proof}

Since $\E[X_i] = r + f (\mu -r)$ and $\E[X_i]^2 = r^2 +  O(\mu^3)$,
$$
\E[\log(1+X_i)] = \E[X_i] - \frac{\V[X_i]}{2} - \frac{r^2}{2} + O(\mu^3),
$$
so
$$
\E[\log(1+X_i)] = r - \frac{r^2}{2} + f(\mu -r) - f^2 \frac{\sigma^2}{2}  + O(\mu^3).
$$

Hence
$$
f^* = \frac{\mu -r}{\sigma^2}
$$
gives an approximation $f^* = f_\text{max} + O(\mu^2)$, and it satisfies
$$
\E[\log(1+X_i(f^*))] = \frac{S^2}{2} + r - \frac{r^2}{2}+ O(\mu^3)
$$
for $S = \frac{\mu -r}{\sigma}$.

\section{Proof for alternative approximation formula for Section \ref{OptimalF} (to be removed before release}

This section gives a previous version of the proofs of the approximation formula for $\E[\log(1+X_i)]$.
\memo{
It shows exactly the same equations as described in \cite{Thorp2006}, but it requires $c$ to be small as well as $\mu$, with an extra constraints to $\mu$ and $c$.  In reality $c$ can be a non-small number compared with $\mu$, so I would like to replace it with those in the previous section.
}

First, we can write the optimal $f$ explicitly:

\begin{align*}
\E[\log(1+ X_i)] &= p_i \log(1 + (1-f) r + f u_i) + (1-p_i)\log(1+ (1-f)r + f d_i)
\end{align*}
%\frac{M_{i}\,\log\left(-\frac{\left(M_{i}\,f-M_{i}\right)\,r+\left(M_{i}\,c-B\right)\,f-M_{i}}{M_{i}}\right)}{M_{i}+M_{-i}} +\frac{M_{-i}\,\log\left(\left(1-f\right)\,r-c\,f+1\right)}{M_{i}+M_{-i}}
for
$$
p_i = \frac{M_i}{M_i + M_{-i}},
$$
$$
u_i = \frac{B}{M_i} - c,
$$
and
$$
d_i = -c.
$$
By a straight-forward calculus we obtain
\begin{align*}
     f_\text{max} & =\frac{M_{i}\,\left(r+1\right)\,\left( (M_i + M_{-i}) (c+r)-B\right)}{\left(M_{-i}+M_{i}\right)\,\left(r+c\right)\,\left(M_{i}\,(r+c)-B\right)}.
\end{align*}


Let
$$
\mu = \frac{B}{M_i + M_{-i}} -  c.
$$
We approximate $f_\text{max}$ and $\E[\log(1+X_i)]$ when $\mu$ is small.
By eliminating $M_i$ we obtain
\begin{align*}
f_\text{max} &= \frac{ \left(B- M_{-i}\,(\mu+c) \right)\,\left(r+1\right)\,\left(\mu-r\right)}{\left(c+r\right)\,\left(M_{-i}\,(\mu + c) (c + r) +B\,(\mu - r)\right)}.
\end{align*}
so we have this lemma.
\begin{lemma}
If $0 < r < \mu$, then
\begin{align*}
    f_\text{max} &< \frac{B (r+1) (\mu -r)}{M_{-i} c^3}.
\end{align*}
\end{lemma}

We are interested in $f$ that maximizes the log-return, so we assume $f_\text{max} = O(c^{-3}\mu)$ as $c, r, \mu \to 0$.

\begin{prop}
Assuming $0< r <\mu < c^4$ and $f = O(c^{-3} \mu)$ as $c, r, \mu \to 0$, we claim approximation
$$
\E[\log(1+X_i)] = \E[X_i] - \frac{\E[X_i^2]}{2} + O(\mu^2)
$$
as $c, r, \mu \to 0$.
\end{prop}
\begin{proof}
Since $\log(1+x) -( x - \frac{x^2}{2}) < \frac{x^3}{3}$ for all $x> -1$, we have
$\E[\log(1+X_i)] - (\E[X_i] - \frac{\E[X_i^2]}{2}) < \E[X_i^3],$
so it suffices to show $\E[X_i^3]= O(\mu^2)$.
Since $f = O(c^{-3}\mu)$ and $0 < r< \mu$,
there exists $C=C(M_{-i})$ that satisfies
\begin{align*}
    \E[X_i^3] &= p_i ( (1-f) r + f u_i)^3 + (1-p_i) ( (1-f)r + f d_i)^3\\
    &\le  C c^5 (c^{-3}\mu)^3\\
    &\le  C \mu^2
\end{align*}
for sufficiently small $\mu$ because for
$$D_3 = M_{2}^2\,r^2+\left(2\,M_{2}^2\,\left(\mu-r\right)+2\,M_{2}^2\,c-2\,B\,M_{2}\right)\,r+\left(2\,M_{2}^2\,c-2\,B\,M_{2}\right)\,\left(\mu-r\right)+M_{2}^2\,\left(\mu-r\right)^2+M_{2}^2\,c^2-2\,B\,M_{2}\,c+B^2$$
and
$$D_2 = B- M_{2}\,r-M_{2}\,\left(\mu-r\right)-M_{2}\,c,$$
\begin{align*}
\E[X_i^3] &= \frac{f^3}{D_3}\{ \left(2\,M_{2}^2\,r^5+\left(7\,M_{2}^2\,\left(\mu-r\right)+10\,M_{2}^2\,c-B\,M_{2}\right)\right)\,r^4\\
& + \left(\left(28\,M_{2}^2\,c-B\,M_{2}\right)\,\left(\mu-r\right)+8\,M_{2}^2\,\left(\mu-r\right)^2+20\,M_{2}^2\,c^2-4\,B\,M_{2}\,c\right)r^3\\
&+\left(\left(42\,M_{2}^2\,c^2-3\,B\,M_{2}\,c\right)\,\left(\mu-r\right)+3\,M_{2}^2\,\left(\mu-r\right)^3+\left(24\,M_{2}^2\,c+3\,B\,M_{2}\right)\,\left(\mu-r\right)^2+20\,M_{2}^2\,c^3-6\,B\,M_{2}\,c^2\right)r^2\\
&+\left(\left(28\,M_{2}^2\,c^3-3\,B\,M_{2}\,c^2\right)\,\left(\mu-r\right)+\left(6\,M_{2}^2\,c+3\,B\,M_{2}\right)\,\left(\mu-r\right)^3\right)r\\
&+\left(\left(24\,M_{2}^2\,c^2+6\,B\,M_{2}\,c\right)\,\left(\mu-r\right)^2+10\,M_{2}^2\,c^4-4\,B\,M_{2}\,c^3\right)r\\
&+\left(\left(7\,M_{2}^2\,c^4-B\,M_{2}\,c^3\right)\,\left(\mu-r\right)+\left(3\,M_{2}^2\,c^2+3\,B\,M_{2}\,c+B^2\right)\,\left(\mu-r\right)^3+\left(8\,M_{2}^2\,c^3+3\,B\,M_{2}\,c^2\right)\,\left(\mu-r\right)^2\right)\\
&+2\,M_{2}^2\,c^5-B\,M_{2}\,c^4\}\\
& +\frac{f^2}{D_2} \{3\,M_{2}\,r^4+\left(9\,M_{2}\,\left(\mu-r\right)+9\,M_{2}\,c\right)\,r^3+\left(18\,M_{2}\,c\,\left(\mu-r\right)+6\,M_{2}\,\left(\mu-r\right)^2+9\,M_{2}\,c^2\right)\,r^2\\
& +\left(9\,M_{2}\,c^2\,\left(\mu-r\right)+\left(6\,M_{2}\,c+3\,B\right)\,\left(\mu-r\right)^2+3\,M_{2}\,c^3\right)\,r\}\\
& +3\,f\,\left(\mu-r\right)\,r^2  +r^3,
\end{align*}
for $M_i = M_1, M_{-i} = M_2$.
\end{proof}

Thus we have 
$$
\E[\log(1+X_i)] = \E[X_i] - \frac{\E[X_i^2]}{2} + O(\mu^2)
$$
as $c, r, \mu \to 0$.
Since $\E[X_i] = r + f (\mu -r)$ and $\E[X_i]^2 =  O(\mu^2)$,
$$
\E[\log(1+X_i)] = \E[X_i] - \frac{\V[X_i^2]}{2} + O(\mu^2),
$$
so
$$
\E[\log(1+X_i)] = r + f(\mu -r) - f^2 \frac{\sigma^2}{2}  + O(\mu^2).
$$

Hence
$$
f^* = \frac{\mu -r}{\sigma^2}
$$
gives an approximation $f^* = f_\text{max} + O(\mu^{1/2})$, and it satisfies
$$
\E[\log(1+X_i(f^*))] = \frac{S^2}{2} + r + O(\mu^2)
$$
for $S = \frac{\mu -r}{\sigma}$.



